Compressive Acquisition of Dynamic Scenes

Compressive sensing (CS) is a new approach for the acquisition and recovery of sparse signals and images that enables sampling rates significantly below the classical Nyquist rate. Despite significant progress in the theory and methods of CS, little headway has been made in compressive video acquisition and recovery. Video CS is complicated by the ephemeral nature of dynamic events, which makes direct extensions of standard CS imaging architectures and signal models difficult. In this paper, we develop a new framework for video CS for dynamic textured scenes that models the evolution of the scene as a linear dynamical system (LDS). This reduces the video recovery problem to first estimating the model parameters of the LDS from compressive measurements, and then reconstructing the image frames. We exploit the low-dimensional dynamic parameters (the state sequence) and high-dimensional static parameters (the observation matrix) of the LDS to devise a novel compressive measurement strategy that measures only the dynamic part of the scene at each instant and accumulates measurements over time to estimate the static parameters. This enables us to lower the compressive measurement rate considerably. We validate our approach with a range of experiments involving both video recovery, sensing hyper-spectral data, and classification of dynamic scenes from compressive data. Together, these applications demonstrate the effectiveness of the approach.

==> formulation.tex <==
For the rest of the paper, we use the following notation. At time $t$, the image observation (the $t$-th frame of the video)
is $\bfy_t \in {\mathbb R}^{N}$ and the hidden state is $\bfx_t \in {\mathbb R}^d$ such that
$\bfy_t = C \bfx_t$, where $C \in {\mathbb R}^{N \times d}$ is the observation matrix.
We use ${\bf z}$ to denote compressive measurements and $\Phi$ and $\Psi$ to denote the
measurement and sparsifying matrices respectively. We use ``:'' subscripts to denote sequences,
such as $\bfx_{1:T} = \{\bfx_1, \bfx_2, \ldots, \bfx_T\}$ and  $[ \cdot ]_{1:T}$ to denote matrices,
such as $[\bfy]_{1:T}$ is the $N \times T$ matrix formed by $\bfy_{1:T}$ such that the $k$-th column is $\bfy_k$.


